On infinitesimal contraction analysis for hybrid systems

Infinitesimal contraction analysis, wherein global asymptotic convergence results are obtained from local dynamical properties, has proven to be a powerful tool for applications in biological, mechanical, and transportation systems. The technique has primarily been developed for systems governed by a single, possibly nonsmooth, differential or difference equation. We generalize infinitesimal contraction analysis to hybrid systems governed by interacting differential and difference equations. Importantly, we leverage an intrinsic distance function to derive the first contraction results for hybrid systems without restrictions on mode sequence or dwell time. Our theoretical results are illustrated in several examples and applications.

==> elastic.tex <==
\ddot{q}_{\air} &=\left[\begin{matrix}- g + \frac{- \beta \left(\dot{q}_1 - \dot{q}_2\right) + \kappa \left(\eta - q_{1} + q_{2} + u\right)}{m_{1}}\\- g - \frac{- \beta \left(\dot{q}_1 - \dot{q}_2\right) + \kappa \left(\eta - q_{1} + q_{2} + u\right)}{m_{2}}\end{matrix}\right]
\\
\ddot{q}_{\gnd} &=\left[\begin{matrix}- g + \frac{- \beta \dot{q}_1 + \kappa \left(\eta - q_{1} + u\right)}{m_{1}}\end{matrix}\right]
\\
\F_{\air} &=\left[\begin{matrix}\dot{q}_1\\\dot{q}_2\\- g + \frac{- \beta \left(\dot{q}_1 - \dot{q}_2\right) + \kappa \left(\eta - q_{1} + q_{2} + u\right)}{m_{1}}\\- g - \frac{- \beta \left(\dot{q}_1 - \dot{q}_2\right) + \kappa \left(\eta - q_{1} + q_{2} + u\right)}{m_{2}}\end{matrix}\right]
\\
\F_{\gnd} &=\left[\begin{matrix}\dot{q}_1\\- g + \frac{- \beta \dot{q}_1 + \kappa \left(\eta - q_{1} + u\right)}{m_{1}}\end{matrix}\right]
\\
D_x \F_{\air} &=\left[\begin{matrix}0 & 0 & 1 & 0\\0 & 0 & 0 & 1\\- \frac{\kappa}{m_{1}} & \frac{\kappa}{m_{1}} & - \frac{\beta}{m_{1}} & \frac{\beta}{m_{1}}\\\frac{\kappa}{m_{2}} & - \frac{\kappa}{m_{2}} & \frac{\beta}{m_{2}} & - \frac{\beta}{m_{2}}\end{matrix}\right]
\\
D_x \F_{\gnd} &=\left[\begin{matrix}0 & 1\\- \frac{\kappa}{m_{1}} & - \frac{\beta}{m_{1}}\end{matrix}\right]
\\
g_{\LO} &=- \beta \dot{q}_1 + \kappa \left(\eta - q_{1} + u\right) + g m_{2}
\\
\R_{\LO}^\tr &=\left[\begin{matrix}q_{1} & 0 & \dot{q}_1 & 0\end{matrix}\right]
\\
\Xi_{\LO} &=\left[\begin{matrix}1 & 0\\0 & 0\\0 & 1\\0 & 0\end{matrix}\right]
\\
g_{\TD} &=q_{2}
\\
\R_{\TD}^\tr &=\left[\begin{matrix}q_{1} & \dot{q}_1\end{matrix}\right]
\\
\Xi_{\TD} &=\left[\begin{matrix}1 & 0 & 0 & 0\\0 & - \frac{\beta}{m_{1}} & 1 & 0\end{matrix}\right]
\\
e_{\air} &=\frac{\dot{q}_1^{2} m_{1}}{2} + \frac{\dot{q}_2^{2} m_{2}}{2} + \frac{\kappa \left(\eta - q_{1} + q_{2} + u\right)^{2}}{2} + g \left(m_{1} q_{1} + m_{2} q_{2}\right)
\\
e_{\gnd} &=\frac{\dot{q}_1^{2} m_{1}}{2} + \frac{\kappa \left(\eta - q_{1} + u\right)^{2}}{2} + g m_{1} q_{1}
\\
E_{\air} &=\left[\begin{matrix}\kappa & - \kappa & 0 & 0\\- \kappa & \kappa & 0 & 0\\0 & 0 & m_{1} & 0\\0 & 0 & 0 & m_{2}\end{matrix}\right]
\\
E_{\gnd} &=\left[\begin{matrix}\kappa & 0\\0 & m_{1}\end{matrix}\right]
\\
\frac{1}{2}\paren{D_x \F_{\air}^\tr \cdot E_{\air} + E_{\air} \cdot D_x \F_{\air}} &=\left[\begin{matrix}0 & 0 & 0 & 0\\0 & 0 & 0 & 0\\0 & 0 & - \beta & \beta\\0 & 0 & \beta & - \beta\end{matrix}\right]
\\
\frac{1}{2}\paren{D_x \F_{\gnd}^\tr \cdot E_{\gnd} + E_{\gnd} \cdot D_x \F_{\gnd}} &=\left[\begin{matrix}0 & 0\\0 & - \beta\end{matrix}\right]
\\

==> visco.tex <==
\ddot{q}_{\emptyset} &=\left[\begin{matrix}\frac{1}{m_\lft} \left(- \beta_\lft \dot{q}_\lft + \kappa_\lft \left(\eta_\lft - q_\lft\right) - \kappa_\perp \left(\ell + q_\lft - q_\rght\right) - \kappa_\| \left(q_\lft - q_\rght + u\right)\right)\\\frac{1}{m_\rght} \left(\kappa_\perp \left(\ell + q_\lft - q_\rght\right) + \kappa_\| \left(q_\lft - q_\rght + u\right)\right)\end{matrix}\right]
\\
\F_{\emptyset} &=\left[\begin{matrix}\dot{q}_\lft\\\dot{q}_\rght\\- \frac{\kappa_\perp}{\beta} \left(\ell + q_\lft - q_\rght\right)\\\frac{1}{m_\lft} \left(- \beta_\lft \dot{q}_\lft + \kappa_\lft \left(\eta_\lft - q_\lft\right) - \kappa_\perp \left(\ell + q_\lft - q_\rght\right) - \kappa_\| \left(q_\lft - q_\rght + u\right)\right)\\\frac{1}{m_\rght} \left(\kappa_\perp \left(\ell + q_\lft - q_\rght\right) + \kappa_\| \left(q_\lft - q_\rght + u\right)\right)\end{matrix}\right]
\\
D_x \F_{\emptyset} &=\left[\begin{matrix}0 & 0 & 0 & 1 & 0\\0 & 0 & 0 & 0 & 1\\- \frac{\kappa_\perp}{\beta} & \frac{\kappa_\perp}{\beta} & - \frac{\kappa_\perp}{\beta} & 0 & 0\\\frac{1}{m_\lft} \left(- \kappa_\lft - \kappa_\perp - \kappa_\|\right) & \frac{1}{m_\lft} \left(\kappa_\perp + \kappa_\|\right) & - \frac{\kappa_\perp}{m_\lft} & - \frac{\beta_\lft}{m_\lft} & 0\\\frac{1}{m_\rght} \left(\kappa_\perp + \kappa_\|\right) & \frac{1}{m_\rght} \left(- \kappa_\perp - \kappa_\|\right) & \frac{\kappa_\perp}{m_\rght} & 0 & 0\end{matrix}\right]
\\
E_{\emptyset} &=\left[\begin{matrix}\kappa_\lft + \kappa_\perp + \kappa_\| & - \kappa_\perp - \kappa_\| & \kappa_\perp & 0 & 0\\- \kappa_\perp - \kappa_\| & \kappa_\perp + \kappa_\| & - \kappa_\perp & 0 & 0\\\kappa_\perp & - \kappa_\perp & \kappa_\perp & 0 & 0\\0 & 0 & 0 & m_\lft & 0\\0 & 0 & 0 & 0 & m_\rght\end{matrix}\right]
\\
\frac{1}{2}\paren{D_x \F_{\emptyset}^\tr \cdot E_{\emptyset} + E_{\emptyset} \cdot D_x \F_{\emptyset}} &=\left[\begin{matrix}- \frac{\kappa_\perp^{2}}{\beta} & \frac{\kappa_\perp^{2}}{\beta} & - \frac{\kappa_\perp^{2}}{\beta} & 0 & 0\\\frac{\kappa_\perp^{2}}{\beta} & - \frac{\kappa_\perp^{2}}{\beta} & \frac{\kappa_\perp^{2}}{\beta} & 0 & 0\\- \frac{\kappa_\perp^{2}}{\beta} & \frac{\kappa_\perp^{2}}{\beta} & - \frac{\kappa_\perp^{2}}{\beta} & 0 & 0\\0 & 0 & 0 & - \beta_\lft & 0\\0 & 0 & 0 & 0 & 0\end{matrix}\right]
\\
\spec\frac{1}{2}\paren{D_x \F_{\emptyset}^\tr \cdot E_{\emptyset} + E_{\emptyset} \cdot D_x \F_{\emptyset}} &=\left[\begin{matrix}- \beta_\lft & - \frac{3 \kappa_\perp^{2}}{\beta} & 0\end{matrix}\right]
\\
g_{\emptyset,\lft} &=q_\lft
\\
D_t g_{\emptyset,\lft} &=0
\\
D_x g_{\emptyset,\lft} &=\left[\begin{matrix}1 & 0 & 0 & 0 & 0\end{matrix}\right]
\\
R_{\emptyset,\lft} &=\left[\begin{matrix}q_\rght\\\ell\\\dot{q}_\rght\end{matrix}\right]
\\
D_t R_{\emptyset,\lft} &=\left[\begin{matrix}0\\0\\0\end{matrix}\right]
\\
D_x R_{\emptyset,\lft} &=\left[\begin{matrix}0 & 1 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 1\end{matrix}\right]
\\
\Xi_{\emptyset,\lft} &=\left[\begin{matrix}0 & 1 & 0 & 0 & 0\\0 & 0 & 1 & 0 & 0\\0 & 0 & 0 & 0 & 1\end{matrix}\right]
\\
\ddot{q}_{\lft} &=\left[\begin{matrix}\frac{1}{m_\rght} \left(\kappa_\perp \left(\ell - q_\rght\right) + \kappa_\| \left(- q_\rght + u\right)\right)\end{matrix}\right]
\\
\F_{\lft} &=\left[\begin{matrix}\dot{q}_\rght\\- \frac{\kappa_\perp}{\beta} \left(\ell - q_\rght\right)\\\frac{1}{m_\rght} \left(\kappa_\perp \left(\ell - q_\rght\right) + \kappa_\| \left(- q_\rght + u\right)\right)\end{matrix}\right]
\\
D_x \F_{\lft} &=\left[\begin{matrix}0 & 0 & 1\\\frac{\kappa_\perp}{\beta} & - \frac{\kappa_\perp}{\beta} & 0\\\frac{1}{m_\rght} \left(- \kappa_\perp - \kappa_\|\right) & \frac{\kappa_\perp}{m_\rght} & 0\end{matrix}\right]
\\
E_{\lft} &=\left[\begin{matrix}\kappa_\perp + \kappa_\| & - \kappa_\perp & 0\\- \kappa_\perp & \kappa_\perp & 0\\0 & 0 & m_\rght\end{matrix}\right]
\\
\frac{1}{2}\paren{D_x \F_{\lft}^\tr \cdot E_{\lft} + E_{\lft} \cdot D_x \F_{\lft}} &=\left[\begin{matrix}- \frac{\kappa_\perp^{2}}{\beta} & \frac{\kappa_\perp^{2}}{\beta} & 0\\\frac{\kappa_\perp^{2}}{\beta} & - \frac{\kappa_\perp^{2}}{\beta} & 0\\0 & 0 & 0\end{matrix}\right]
\\
\spec\frac{1}{2}\paren{D_x \F_{\lft}^\tr \cdot E_{\lft} + E_{\lft} \cdot D_x \F_{\lft}} &=\left[\begin{matrix}- \frac{2 \kappa_\perp^{2}}{\beta} & 0\end{matrix}\right]
\\
g_{\lft,\emptyset} &=- \frac{1}{m_\lft} \left(\eta_\lft \kappa_\lft - \kappa_\perp \left(\ell - q_\rght\right) - \kappa_\| \left(- q_\rght + u\right)\right)
\\
D_t g_{\lft,\emptyset} &=0
\\
D_x g_{\lft,\emptyset} &=\left[\begin{matrix}- \frac{1}{m_\lft} \left(\kappa_\perp + \kappa_\|\right) & \frac{\kappa_\perp}{m_\lft} & 0\end{matrix}\right]
\\
R_{\lft,\emptyset} &=\left[\begin{matrix}0\\q_\rght\\\ell\\0\\\dot{q}_\rght\end{matrix}\right]
\\
D_t R_{\lft,\emptyset} &=\left[\begin{matrix}0\\0\\0\\0\\0\end{matrix}\right]
\\
D_x R_{\lft,\emptyset} &=\left[\begin{matrix}0 & 0 & 0\\1 & 0 & 0\\0 & 1 & 0\\0 & 0 & 0\\0 & 0 & 1\end{matrix}\right]
\\
\Xi_{\lft,\emptyset} &=\left[\begin{matrix}0 & 0 & 0\\1 & 0 & 0\\0 & 1 & 0\\0 & 0 & 0\\0 & 0 & 1\end{matrix}\right]
\\

==> viscoelastic.tex <==
\F_{air} &=\left[\begin{matrix}\dot{q}_1\\\dot{q}_2\\\frac{\kappa_\perp \left(\ell + \eta_\perp - q_{1} + q_{2}\right)}{m_{1}} - g\\- \frac{\kappa_\perp \left(\ell + \eta_\perp - q_{1} + q_{2}\right)}{m_{2}} - g\\\frac{- \ell \kappa_\parallel - \ell \kappa_\perp + \eta_\parallel \kappa_\parallel - \eta_\perp \kappa_\perp + \kappa_\parallel u + \kappa_\perp q_{1} - \kappa_\perp q_{2}}{\beta}\end{matrix}\right]
\\
\F_{gnd} &=\left[\begin{matrix}\dot{q}_1\\\frac{\kappa_\perp \left(\ell + \eta_\perp - q_{1}\right)}{m_{1}} - g\\\frac{- \ell \kappa_\parallel - \ell \kappa_\perp + \eta_\parallel \kappa_\parallel - \eta_\perp \kappa_\perp + \kappa_\parallel u + \kappa_\perp q_{1}}{\beta}\end{matrix}\right]
\\
g_{LO} &=\kappa_\perp \left(\ell + \eta_\perp - q_{1}\right) + g m_{2}
\\
\R_{LO}^\tr &=\left[\begin{matrix}q_{1} & 0 & \dot{q}_1 & 0 & \ell\end{matrix}\right]
\\
g_{TD} &=q_{2}
\\
\R_{TD}^\tr &=\left[\begin{matrix}q_{1} & \dot{q}_1 & \ell\end{matrix}\right]
\\
e_{air} &=\frac{\dot{q}_1^{2} m_{1}}{2} + \frac{\dot{q}_2^{2} m_{2}}{2} + \frac{\kappa_\parallel \left(- \ell + \eta_\parallel\right)^{2}}{2} + \frac{\kappa_\perp \left(\ell + \eta_\perp - q_{1} + q_{2}\right)^{2}}{2} + g \left(m_{1} q_{1} + m_{2} q_{2}\right)
\\
e_{gnd} &=\frac{\dot{q}_1^{2} m_{1}}{2} + \frac{\kappa_\parallel \left(- \ell + \eta_\parallel\right)^{2}}{2} + \frac{\kappa_\perp \left(\ell + \eta_\perp - q_{1}\right)^{2}}{2} + g m_{1} q_{1}
\\
E_{air} &=\left[\begin{matrix}\kappa_\perp & - \kappa_\perp & 0 & 0 & - \kappa_\perp\\- \kappa_\perp & \kappa_\perp & 0 & 0 & \kappa_\perp\\0 & 0 & m_{1} & 0 & 0\\0 & 0 & 0 & m_{2} & 0\\- \kappa_\perp & \kappa_\perp & 0 & 0 & \kappa_\parallel + \kappa_\perp\end{matrix}\right]
\\
E_{gnd} &=\left[\begin{matrix}\kappa_\perp & 0 & - \kappa_\perp\\0 & m_{1} & 0\\- \kappa_\perp & 0 & \kappa_\parallel + \kappa_\perp\end{matrix}\right]
